Relativistic recoil, electron-correlation, and QED effects on the 2p_j-2s transition energies in Li-like ions

The relativistic nuclear recoil, higher-order interelectronic-interaction, and screened QED corrections to the transition energies in Li-like ions are evaluated. The calculation of the relativistic recoil effect is performed to all orders in 1/Z. The interelectronic-interaction correction to the transition energies beyond the two-photon exchange level is evaluated to all orders in 1/Z within the Breit approximation. The evaluation is carried out employing the large-scale configuration-interaction Dirac-Fock-Sturm method. The rigorous calculation of the complete gauge invariant sets of the screened self-energy and vacuum-polarization diagrams is performed utilizing a local screening potential as the zeroth-order approximation. The theoretical predictions for the 2p_j-2s transition energies are compiled and compared with available experimental data in the range of the nuclear charge number Z=10-60.

==> E3_test_2.tex <==
% \oddsidemargin=-0.6cm \textwidth=17.5cm \topmargin=-1.0cm
% \textheight=24.cm
% \footskip=2.0cm
\begin{table}
\caption{Dlya Proverok. Obshaya dinamika ot $Z$.  The third- and higher-order interelectronic-interaction correction
to the energies of $n=2$ states of Li-like ions, in eV. }
\linespread{1}
\begin{center}
\begin{tabular}{rlcrrrllc}
 \hline
 \hline
$Z$&Interaction&Order of&$2s$&$2p_{1/2}$&$2p_{3/2}$&$2p_{1/2}$&$2p_{3/2}$\\
   &           &Interaction&   &          &          &   $-2s$&   $-2s$     
\\

 \hline
 \hline
     3&C+B  &$E_3$&-0.1518  &-0.6368  &-0.6384  &-0.4850(2)(0)  &-0.4866(2)(0)
&[TW ]\\
     3&C+B  &$E_{\geqslant 3}$&-0.3627  &-1.0116  &-1.0132  &-0.6489(2)(0) 
&-0.6505(2)(0)  &[TW ]\\
 \hline
 \hline
    30&C    &$E_3$&-0.0098  &-0.0504  &-0.0609  &-0.0406  &-0.0511 &[TW]\\
    30&C    &$E_3$& &  &  &-0.0450  &   &[ZherO]\\
    30&C    &$E_{\geqslant 3}$&-0.0111  &-0.0529  &-0.0629  &-0.0418 &-0.0518 &[TW]\\
    30&C    &$E_{\geqslant 3}$&  & &   &-0.0460  &   &[ZherO]\\
 \hline
    30&C+B &$E_3$& 0.0157  &-0.0129  &-0.0314  &-0.0287(3)(1) 
&-0.0471(3)(1) &[TW]\\
    30&C+B  &$E_3$& &  &  &-0.0360  &   &[ZherO]\\
    30&C+B  &$E_3$&   &  &  &-0.0278 &-0.0463 &[Yer]\\
    30&C+B  &$E_3$&   &  &  &-0.060 & &[Andr]\\
    30&C+B  &$E_3$&   &  &  &-0.030 & &[Andr2]\\

    30&C+B &$E_{\geqslant 3}$& 0.0140  &-0.0159  &-0.0339  &-0.0299(3)()
&-0.0479(3)() &[TW]\\
    30&C+B  &$E_3$& &  &  &-0.0360  &   &[ZherO]\\
 \hline
 \hline 
    60&C+B  &$E_3$& 0.0676  & 0.1006  & 0.0437  & 0.0328(10)(10) 
&-0.0235(10)(10) &[Kozh ]\\
    60&C+B  &$E_3$&   &   &  & 0.0330  &  &[ZherN]\\
    60&C+B  &$E_3$&  &  &   & 0.0430  &  &[Andr ]\\
    60&C+B  &$E_3$&  &  &   & 0.035  &  &[And2 ]\\
    60&C+B  &$E_{\geqslant 3}$& 0.0666  & 0.0985  & 0.0425  & 0.0319(10)(10) 
&-0.0238(10)(10)  &[Kozh ]\\
 \hline
 \hline
    83&C    &$E_3$& 0.0264  & 0.0592  & 0.0003  & 0.0328  &-0.0261  &[Kozh ]\\
    83&C    &$E_3$&   &  &  & 0.0310  &  &[ZherN]\\
    83&C    &$E_{\geqslant 3}$& 0.0261  & 0.0573  &-0.0014  & 0.0312  &-0.0275  &[Kozh ]\\
 \hline
    83&C+B  &$E_3$& 0.1321  & 0.2307  & 0.1041  & 0.098(5)(10) 
&-0.030(5)(10)  &[Kozh ]\\
    83&C+B  &$E_3$&  &   &   & 0.104  &  &[ZherN]\\
    83&C+B  &$E_3$&   &  &  &0.103 &-0.019 &[Yer]\\
    83&C+B  &$E_{\geqslant 3}$& 0.1302  & 0.2283  & 0.1028  & 0.097(5)(10) 
&-0.029(5)(10)  &[Kozh ]\\
 \hline
 \hline
    92&C+B  &$E_3$& 0.1775  & 0.3158  & 0.1366  & 0.137(7)(300) 
&-0.041(7)(300) &[Kozh ]\\
    92&C+B  &$E_3$&   &   &   & 0.1600  &  &[ZherN]\\
    92&C+B  &$E_3$&   &   &   & 0.1670  &  &[Andr ]\\
    92&C+B  &$E_3$&   &   &   & 0.147  &  &[And2 ]\\
    92&C+B  &$E_{\geqslant 3}$& 0.1739  & 0.3121  & 0.1348  & 0.137(7)(300) 
&-0.039(7)(300)  &[Kozh ]\\
 \hline
 \hline 
\end{tabular}
\end{center}
\end{table}


==> E_int_2.tex <==

\begin{table}
\caption{Electronic-structure contributions 
to the $(1s)^22p_{3/2}-(1s)^22s$ and $(1s)^22p_{1/2}-(1s)^22s$ transition energies of lithium,
 in eV.(Pogreshnost' kazhdogo chisla Yer $0.00015$)}
\label{table:E3_Li}
\linespread{1}
 \label{table:E3_Li}
\begin{center}
\begin{tabular}{lrrr}

\hline
\hline
& TW & Yer(Coul) & Yer(LDF)                            \\
\hline
$2p_{1/2}-2s_{1/2}$ transition:& \\
Dirac:          & 0      & 0      &  1.8324 \\
1-phot:         & 5.7775 & 5.7775 & -0.0212 \\
2-ph:     &-3.2803 &-3.2822 &  0.0378\\
3-ph:     &-0.4850 &-0.4816 & -0.0027\\
$_>3$-ph: &-0.1639 &       &  \\
Sum:            & 1.8483 & 2.0136 &  1.8466\\
Exact:          & &1.8481164\\

$2p_{3/2}-2s_{1/2}$ transition:& \\
Dirac:          & 0.0037 & 0.0037 &  1.8324\\
1-phot:         & 5.7690 & 5.7691 & -0.0210      \\
2-ph:     &-3.2738 &-3.2757 &  0.0376\\
3-ph:     &-0.4866 &-0.4841 & -0.0027\\
$_>3$-ph: &-0.1639 &       &  \\
Sum:            & 1.8484 & 2.0128 &  1.8466\\
Exact:          & &1.8481577\\


\end{tabular}
\end{center}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}
\caption{Electronic-structure contributions 
to the $(1s)^22p_{3/2}-(1s)^22s$ and $(1s)^22p_{1/2}-(1s)^22s$ transition energies of Li-like Zn $(Z=30)$,
 in eV.(Pogreshnost' kazhdogo chisla Yer $0.00015$)}
\label{table:E3_Zn}
\linespread{1}
 \label{table:E3_Li}
\begin{center}
\begin{tabular}{lrrr}

\hline
\hline
& TW & Yer(Coul) & Yer(LDF)                            \\
\hline
$2p_{1/2}-2s_{1/2}$ transition:& \\
Dirac:          & -0.0143 & -0.0144 & 56.4876 \\
1-phot:         & 62.1468 & 62.1467 & 1.5701 \\
2-ph(Breit): & -3.8907 & -3.8910 & 0.1573\\
2-ph(QED):       &  0.0014 &0.0014& 0.0011\\ 
3-ph(Breit):     & -0.0287 & -0.0278& -0.0030\\
$_>3$-ph(Breit): & -0.0012 &      &  \\
Sum:            & 58.2133 & 58.2152 & 58.2130 \\


$2p_{3/2}-2s_{1/2}$ transition:& \\
Dirac:          & 37.7992 & 37.7991 & 87.0030\\
1-phot:         & 53.2346 & 53.2344 & 0.7353      \\
2-ph(Breit): & -3.1949 & -3.1982 & 0.0495\\
2-ph(QED): & 0.0027 & 0.0060 & 0.0052\\
3-ph(Breit):     & -0.0471 & -0.0463 &-0.0003 \\
$_>3$-ph(Breit): & -0.0008 &       &  \\
Sum:            & 87.7937 & 87.7951 & 87.7926 \\



\end{tabular}
\end{center}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}
\caption{Electronic-structure contributions 
to the $(1s)^22p_{3/2}-(1s)^22s$ and $(1s)^22p_{1/2}-(1s)^22s$ transition energies of Li-like Bi $(Z=83)$,
 in eV.(Pogreshnost' kazhdogo chisla Yer $0.0015$)}
\label{table:E3_Bi}
\linespread{1}
 \label{table:E3_Li}
\begin{center}
\begin{tabular}{lrrr}

\hline
\hline
& TW & Yer(Coul) & Yer(LDF)      \\
\hline
$2p_{1/2}-2s_{1/2}$ transition:& \\
Dirac:          & -11.898 & -11.900 & 231.974 \\
1-phot:         & 286.678 & 286.680 &  32.085\\
2-ph(Breit): & -10.564 & -10.484 & 0.343\\
2-ph(QED): & 0.116 &  0.038& 0.035\\
3-ph(Breit):     & 0.109(5) & 0.103& -0.008\\
$_>3$-ph(Breit): & -0.002 &      &  \\
Sum:            & 264.433 & 264.435 & 264.427 \\


$2p_{3/2}-2s_{1/2}$ transition:& \\
Dirac:          & 2792.208 & 2792.206 & 2815.692\\
1-phot:         & 23.818 & 23.818 &   -1.540 \\
2-ph(Breit): & -1.804 & -1.918 & -0.057\\
2-ph(QED): & 0.199 & 0.315 & 0.302\\
3-ph(Breit):     & -0.020(5) & -0.019 & -0.005\\
$_>3$-ph(Breit): & -0.001 &       &  \\
Sum:            & 2814.401 & 2814.403 & 2814.392 \\



\end{tabular}
\end{center}
\end{table}

